The Spotlight: A General Method for Discovering Systematic Errors in Deep Learning Models

Supervised learning models often make systematic errors on rare subsets of the data. When these subsets correspond to explicit labels in the data (e.g., gender, race) such poor performance can be identified straightforwardly. This paper introduces a method for discovering systematic errors that do not correspond to such explicitly labelled subgroups. The key idea is that similar inputs tend to have similar representations in the final hidden layer of a neural network. We leverage this structure by "shining a spotlight" on this representation space to find contiguous regions where the model performs poorly. We show that the spotlight surfaces semantically meaningful areas of weakness in a wide variety of existing models spanning computer vision, NLP, and recommender systems.

==> sections/acknowledgements.tex <==
This work was supported by Compute Canada, a GPU grant from NVIDIA, an NSERC Discovery Grant, a DND/NSERC Discovery Grant Supplement, a CIFAR Canada AI Research Chair at the Alberta Machine Intelligence Institute, and DARPA award FA8750-19-2-0222, CFDA \#12.910, sponsored by the Air Force Research Laboratory.
Addtionally, resources used in preparing this research were provided, in part, by NSERC, the Province of Ontario, the Government of Canada through CIFAR, and companies sponsoring the Vector Institute \url{www.vectorinstitute.ai/\#partners}.

==> sections/checklist.tex <==
\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{We will include our code in the supplemental material.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{In Section~\ref{sec:experiments}, we discuss our choice of spotlights.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNo{Our results are qualitative in nature.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{We describe the compute resources that we used in Section~\ref{sec:experiments}.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{In Section~\ref{sec:experiments}, we cite sources for the datasets and models that we study.}
  \item Did you mention the license of the assets?
    \answerYes{In Appendix~\ref{sec:datasets}}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{We will include our code in the supplemental material.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNo{We use pre-existing, publicly available datasets.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{In Appendix~\ref{sec:datasets}}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

==> sections/rough_results_kernel.tex <==

fairface

imagenet
- 1: clutter
- 2: ?
- 3: plants/animals in foliage 
- 4: food; person holding 1 object
- 5: dogs (and suits?)

amazon: 
- spotlight 1: spanish
- spotlight 2: long novel reviews
- spotlight 3: customer service 

movielens
- spotlight 1: sci-fi/adventure; movies with moderate number of reviews; users with lots of reviews; model uncertain over all 5 reviews
- spotlight 2: film-noir/war; users with few reviews (repeated!); model certain review isn't a 1
- spotlight 3: horror/action/adventure leaning; users with many reviews on movies with very few reviews; model certain review isn't a 5


